A model for the current-voltage characteristic of membrane/electrolyte junctions

A model for the current-voltage characteristic of the junction between an Ion-Sensitive-Membrane and an electrolyte solution is derived and compared with numerical simulations of the Poisson-Nernst-Planck model for ion transport. The expression resembles that of a semiconductor pn junction with a non-ideality factor of 2. The non-ideality correlated to the voltage drop in the electrolyte induced by the re-arrangement of the counter-ions.

==> APL_instructions.tex <==
Applied Physics Letters (APL) is an international, peer-reviewed letters journal publishing concise papers in all areas of applied physics that communicate original research discoveries justifying rapid publication.

Cover Letter
\textbf{Authors submitting to APL are encouraged to provide a cover letter as part of their submission.}

It can help convey the importance of the research to the Editors, explain why you consider the paper appropriate for the broad readership of Applied Physics Letters, and specifically how it aligns with the criteria for publication.
The cover letter should make a clear statement on the manuscript’s significance and list related work by the authors.
This letter will not be shared with reviewers. It is intended to aid in the editorial pre-screening of manuscripts.

Manuscript Information:

Article Length

At the time of initial submission, your paper needs to be \textbf{3000 words or less, including figure and table captions.} This word count excludes the title, author list, abstract, acknowledgments, data availability statement, references, and non-text items including figures, tables, and equations.
Normally, papers longer than 3000 words will be rejected, and the authors will be required to shorten the paper and submit it again as a new manuscript.
Longer papers may be considered only in exceptional cases if the quality warrants special consideration. Authors will need to explain the need for the additional length in their cover letter.

Use of Figures
Authors are encouraged to include \textbf{up to five figures in the paper} to illustrate their results.

Images may be grouped together as separate panels in one figure if they are logically connected and clear to the reviewer and readers.

Use of Section Headings
Section heading are not permitted in Letters
